A Theory of Unsupervised Speech Recognition

Unsupervised speech recognition (ASR-U) is the problem of learning automatic speech recognition (ASR) systems from unpaired speech-only and text-only corpora. While various algorithms exist to solve this problem, a theoretical framework is missing from studying their properties and addressing such issues as sensitivity to hyperparameters and training instability. In this paper, we proposed a general theoretical framework to study the properties of ASR-U systems based on random matrix theory and the theory of neural tangent kernels. Such a framework allows us to prove various learnability conditions and sample complexity bounds of ASR-U. Extensive ASR-U experiments on synthetic languages with three classes of transition graphs provide strong empirical evidence for our theory (code available at cactuswiththoughts/UnsupASRTheory.git).

==> bkp/finite_sample_learning_1_12_2023.tex <==
    \paragraph{Matched setup} Now we show that the requirement for distinct eigenvalues is a mild one as it can easily be satisfied with \emph{random} transition matrices. According to such a result, ASR-U is feasible with high probability in the (empirically) \emph{matched} setting commonly used in the ASR-U literature, where the \emph{empirical} generated and true distributions can be matched exactly by some generator in the function class~\cite{Liu2018-asru}. Our proof relies crucially on the seminal work of \cite{NguyenTaoVu2015}.
    \begin{theorem}{(Theorem 2.6 of \cite{NguyenTaoVu2015})}\label{thm:eigenval_gap_symmetric_matrix}
    For any real symmetric matrix of the form $W_n = F_n + X_n$, where $F_n \in \sR^{n\times n}$ is a deterministic symmetric matrix with eigenvalues of order $O(n^\gamma)$ and $X_n$ is a zero-mean, subgaussian random matrix, we have for any $C > 0$, there exists $B > \max\{5\gamma' C + 3\gamma' + 3, 3\gamma'+3\}$ s.t.
    \begin{align*}
        \max_{1\leq i \leq n-1}\Pr[|\lambda_i-\lambda_{i+1}| \leq n^{-B}]\leq n^{-C},
    \end{align*}
    with probability at least $1-O(\exp(-\alpha_0 n))$ for some $\alpha_0 > 0$ dependent on $B$ and $\gamma'=\max\{\gamma, 1/2\}$.
    \end{theorem}
    In the context of ASR-U, it is of particular interest to study the eigenvalue gaps of a Markov random matrix, which unlike the symmetric case, is asymmetric with correlated entries. Fortunately, by modifying the proof for Theorem~\ref{thm:eigenval_gap_symmetric_matrix} we can show that if the language model belongs to a special but rather broad class of Markov random matrices defined below and the states are \emph{non-overlapping} $N$-gram instead of the more common overlapping ones, it should have at least $|\sX|$ distinct eigenvalues with minimum spacing depending on $|\sX|$ and the $N$ for the $N$-gram.

    \begin{definition}{(\smrm/)}
    A \smrm/ is a matrix of the form $A := D^{-1}W$, where the \emph{adjacency matrix} $W$ is a real, symmetric random matrix with positive entries and bounded variance and $D$ is a diagonal matrix with $d_{ii}=\sum_{j} W_{ij} > 0$.
    \end{definition}
    Intuitively, a \smrm/ is the transition matrix for a \textit{reversible} Markov chain formed by normalizing edge weights of a weighted, undirected graph.
    \begin{theorem}{(simple spectrum of \smrm/)}\label{thm:simple_spectrum}
    For any real \smrm/ $A_n = D_n^{-1}W_n \in \sR^{n\times n}$ with adjacency matrix $W_n=F_n+X_n$, where $F_n$ is a deterministic symmetric matrix with eigenvalues of order $n^{\gamma}$ and $X_n$ is a
    symmetric random matrix of zero-mean, unit variance sub-Gaussian random variables,
    %zero-mean, symmetric \subg/ random matrix,
    we have for any $C > 0$, there exists $B > \max\{4\gamma' C+7\gamma'+1, 2C+5\}$ such that
    \begin{align*}
        \max_{1\leq i \leq n-1}\Pr[|\lambda_i-\lambda_{i+1}| \leq n^{-B}]\leq n^{-C},
    \end{align*}
    with probability at least $1-O(\exp(-\alpha_0 n))$ for some $\alpha_0 > 0$ dependent on $B$ and $\gamma'=\max\{\gamma, 1/2\}$.
    \end{theorem}
    %MH: following paragraph is not necessarily true, because $d_{ii}$ may be larger than O(n)
    %Note that compared to Theorem~\ref{thm:eigenval_gap_symmetric_matrix}, the eigenvalue gap for a \smrm/ is in average smaller by at least an order of $n^{-1}$, which is because the normalization factor $d_{ii}$ is of order $O(n)$.
    \begin{corollary}\label{col:simple_spectrum}
    Suppose the speech feature transition probability is a \smrm/ $A := D^{-1}W$ with entries $W_{ij}\sim \mathrm{Uniform}(0, 2\sqrt{3})$ and $D$ is a diagonal matrix with $d_{ii}=\sum_{j}W_{ij}$, then for any $\epsilon > 0$, there exists $\alpha_0 > 0$ such that with probability at least $1-O\left(|\sX|^{-CN}+\exp\left(-\alpha_0|\sX|^N\right)\right)$, the transition probability matrix $A$ has $|\sX|^N$ distinct eigenvalues with minimum gap $|\sX|^{-BN} > 0$.
    \end{corollary}
    The proof of Theorem~\ref{thm:simple_spectrum} and Corollary~\ref{col:simple_spectrum} are presented in detail in the Appendix~\label{appendix:proofs_finite_sample}. 
    
    \paragraph{Unmatched setup} In the finite-sample, unmatched setup, the empirical distribution of the fake text data generated by the GAN does not necessarily match the empirical distribution of the true text data. Assuming the discriminator is perfect in the sense that it
    maintains \Eqref{eq:gan_objective} non-negative, and assuming $D(Y)$ is a scalar random variable, then minimizing \Eqref{eq:gan_objective} is equivalent to minimizing a
    %maximize \Eqref{eq:gan_objective} with respect to any generator $G$, then the GAN boils down to finding an assignment matrix $O$ such that certain
    \emph{divergence measure} $d(\cdot, \cdot)$, between the empirical text distribution, $P^Y$, and the text distribution generated by $O_x(y)=\hat{P}_{Y|X}(y|x)$:
    \begin{align}\label{eq:discrete_perfect_discriminator}
        %\min_{O\in \Delta^{|\sX|\times |\sY|}} d^{\gamma}(\hat{P}_Y,\hat{P}_{X} \circ O),
        \min_{O\in \Delta^{|\sX|\times |\sY|}} d^{\gamma}(P^Y,P^{X} O),
    \end{align}
    where $\gamma > 0$. For example, for the original GAN, $d(\cdot,\cdot)$ is the Jensen-Shannon distance and for the MMD GAN, $d(\cdot, \cdot)$ is the $L_\gamma$ distance between the expectations $\mathbb{E}[D(Y)]$ under the distributions $P^Y$ and $P^XO$.  
    In both cases, Theorem 1 requires \Eqref{eq:discrete_perfect_discriminator} to be the distance between distributions over random sequences, $y=[y_0,\ldots,y_{N(|\mathbb{X}|-1)}]$ of length at least $(|\mathbb{X}|-1)$.  In both cases, however, \Eqref{eq:discrete_perfect_discriminator} can be minimized using a \emph{decomposable} discriminator under the condition that the decomposable discriminator is in the domain space of $(P^y-P^XO)$, where the decomposable discriminator is defined to be:
    \begin{align}\label{eq:decomposable_discrim}
       \E_{Y\sim P_Y}[a(D(Y))] &= \sum_{l=0}^{L-1} \E_{Y\sim P_Y}[a(D_l(Y_l))]\\
       \E_{X\sim P_X}[b(D(G(X)))] &= \sum_{l=0}^{L-1}\E_{X\sim P_X}[b(D_l(G_l(X))],
    \end{align}
    %L2 distance, with $\gamma=2$ in both cases. In the case when $d$ is a distance metric, by Jensen's inequality, we then have 
    %\begin{multline}\label{eq:distance_bound}
    %    d^{\gamma}(\hat{P}_Y,\hat{P}_{X} \circ O) \geq\\ L^\gamma|\sX|^{\gamma(L-1)}d^\gamma\left(\hat{P}^Y,\hat{P}^X  O\right),
    %\end{multline}
    %where equality can be achieved when the discriminator is \emph{decomposable} in the sense that
    %\begin{align}\label{eq:decomposable_discrim}
    %    a_D(y) &= \sum_{l=1}^L a_{D_l}(y_l)\\
    %    b_D(y) &= \sum_{l=1}^L b_{D_l}(y_l),
    %\end{align}
    with \emph{components} $D_l:|\sY|\mapsto \sR,l=1,\cdots,L$. Under the assumption that $D$ is decomposable and that the MMD GAN is used, we have the following sample complexity bound on perfect \asru/.
    % Since the text data $Y_{1:N}$ is discrete in nature, we can estimate $P_{Y_{1:N}}$ to be arbitrarily close to the true distribution \emph{uniformly} given enough samples. As a result, we have
    % \begin{align}
    %   \|\hat{P}^X-P^X\|_1 &\leq \epsilon_X,\\
    %   \|\hat{P}^Y-P^Y\|_1 &\leq \epsilon_Y,
    % \end{align}
    % for the number of speech $N$-grams $n_X$ and the number of text $N$-grams $n_Y$ large enough. Suppose the model is able to minimize \eqref{eq:discrete_perfect_discriminator}, the empirical risk minimizer (ERM) will need to satisfy
    % \begin{align}\label{eq:finite_sample_asr_u}
    %    \hat{P}^X \hat{O} = \hat{P}^Y. 
    % \end{align}
    \begin{theorem}\label{thm:discrete_gan_unsup_asr}
    The empirical risk minimizer (ERM) of \Eqref{eq:discrete_perfect_discriminator} recovers the true assignment $O$ perfectly from $n^X$ speech frames and $n^Y$ text characters with probability $1-2\delta$ if 
    \begin{align*}
        \sigma_{\min}(P^X) \geq
        &\sqrt{\frac{4L|\mathbb{Y}|(n^X+n^Y)+L|\mathbb{X}|n^X}{n^Xn^Y}}+\\
        &10\sqrt{\frac{L\log \frac{1}{\delta}}{n^X\wedge n^Y}},
        %\sigma_{\min}(P^X) \geq \frac{3}{\sqrt{n^X}}+\frac{2}{\sqrt{n^Y}}+10\sqrt{\frac{L\log \frac{1}{\delta}}{n^X\wedge n^Y}},
    \end{align*}
    where $n^X\wedge n^Y := \min\{n^X, n^Y\}$.
    \end{theorem}


==> bkp/preliminary.tex <==
Throughout the paper, we use $P_{X}$ to represent the probability density function (pdf) or probability mass function (pmf) of $X$ depending on the context. For function composition, we denote  $f_g(x)=f(g(x))$. 

